PROOFTOOL: a GUI for the GAPT Framework

This paper introduces PROOFTOOL, the graphical user interface for the General Architecture for Proof Theory (GAPT) framework. Its features are described with a focus not only on the visualization but also on the analysis and transformation of proofs and related tree-like structures, and its implementation is explained. Finally, PROOFTOOL is compared with three other graphical interfaces for proofs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{C. Kaliszyk and C. L\"uth (Eds.): 10th International Workshop\\
on User Interfaces for Theorem Provers\\
EPTCS 118, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.118.1}{10.4204/EPTCS.118.1}}
\pdfoutput=1

